Characterizing Continual Learning Scenarios and Strategies for Audio Analysis

Audio analysis is useful in many application scenarios. The state-of-the-art audio analysis approaches assume the data distribution at training and deployment time will be the same. However, due to various real-life challenges, the data may encounter drift in its distribution or can encounter new classes in the late future. Thus, a one-time trained model might not perform adequately. Continual learning (CL) approaches are devised to handle such changes in data distribution. There have been a few attempts to use CL approaches for audio analysis. Yet, there is a lack of a systematic evaluation framework. In this paper, we create a comprehensive CL dataset and characterize CL approaches for audio-based monitoring tasks. We have investigated the following CL and non-CL approaches: EWC, LwF, SI, GEM, A-GEM, GDumb, Replay, Naive, Cumulative, and Joint training. The study is very beneficial for researchers and practitioners working in the area of audio analysis for developing adaptive models. We observed that Replay achieved better results than other methods in the DCASE challenge data. It achieved an accuracy of 70.12% for the domain incremental scenario and an accuracy of 96.98% for the class incremental scenario.

==> old_5_result_tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[htbp!]
% \caption{Literature for continual learning}
% \scalebox{0.9}{
\begin{table*}[htbp!]
\caption{Comparison of different approaches for \textbf{domain incremental scenario}.}
\centering

\label{tab:DIL}

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\bf Approach    & \textbf{BWT\cite{diaz2018don}} & \textbf{FWT\cite{diaz2018don}} & \textbf{A\cite{diaz2018don}} & \st{OverallAcc.} & \textbf{ACC~\cite{lopez2017gradient}} \\ \hline
EWC            & -4.87             & 62.90             & 65.42                    & 62.83                 & 69.32                  \\ \hline
LwF            & -1.78             & 64.17              & 66.09                    & 62.91                 & 68.78                  \\ \hline
SI             & -2.21             & 60.70              & 62.79                    & 60.96                 & 66.70                  \\ \hline
GDumb          & -2.27              & 57.24              & 57.61                    & 56.32                 & 56.91                  \\ \hline
Replay         & -1.83             & 65.09             & 66.40                    & 62.82                 & 68.16                  \\ \hline
GEM            & -3.53             & 63.21             & 64.94                    & 62.67                 & 67.72                  \\ \hline
Naive          & -5.02             & 62.30            & 64.49                    & 61.50                 & 66.91                  \\ \hline
Cumulative     & 0.76               & 68.35              & 68.82                    & 64.70                 & 71.37                  \\ \hline
Joint  & --                   & --                   & 65.78                    & 73.85                 & 73.85                  \\ \hline
\end{tabular}

\end{table*}
% \begin{table*}[htbp!]
% \caption{Comparative analysis of different CL approaches for domain incremental scenario.}
% \scalebox{1}{
% \label{tab:DIL}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% {\color[HTML]{333333} \textbf{CL strategy}}                   & {\color[HTML]{333333} \textbf{BWT[Diaz]}} & \textbf{BWT[Lopez]} & \textbf{FWT[Diaz]} & \textbf{FWT[Lopez]} & \textbf{Accuracy\cite{diaz2018don}} & \textbf{Overall avg. acc.} & \textbf{\begin{tabular}[c]{@{}l@{}}Last row avg. acc.\end{tabular}} \\ \hline
% \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{EWC}}   & {\color[HTML]{333333} -4.8687}             & 53.61               & 62.8987             & -52.00              & 65.42               & 62.83                      & 69.32                                                                          \\ \hline
% {\color[HTML]{333333} \textbf{LwF}}                           & {\color[HTML]{333333} -1.7827}             & 54.18               & 64.136              & -53.60              & 66.09               & 62.91                      & 68.78                                                                          \\ \hline
% {\color[HTML]{333333} \textbf{SI}}                            & {\color[HTML]{333333} -2.2073}             & 50.15               & 60.696              & -49.90              & 62.79               & 60.96                      & 66.70                                                                          \\ \hline
% \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{GDumb}} & {\color[HTML]{333333} -2.268}              & 49.45               & 57.236              & -48.25              & 57.61               & 56.32                      & 56.91                                                                          \\ \hline
% \textbf{Replay}                                               & -1.8313                                    & 55.31               & 65.0927             & -54.87              & 66.40               & 62.82                      & 68.16                                                                          \\ \hline
% \textbf{GEM}                                                  & -3.5293                                    & 53.43               & 63.2087             & -52.14              & 64.94               & 62.67                      & 67.72                                                                          \\ \hline
% \textbf{Naive}                                                & -5.0193                                    & 53.50               & 62.3047             & 51.56               & 64.49               & 61.50                      & 66.91                                                                          \\ \hline
% \textbf{Cumulative}                                           & 0.764                                      & 56.56               & 68.352              & 57.41               & 68.82               & 64.70                      & 71.37                                                                          \\ \hline
% \textbf{Joint Training}                                       & 0                                          & 0                   & 0                   & 0                   & 65.78               & 73.85                      & 73.85                                                                          \\ \hline
% \end{tabular}
% }
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp!]
\caption{Comparison of different approaches for the \textbf{class incremental scenario}.}
 \label{tab:CIL}
 \centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Approach}    & \textbf{BWT\cite{diaz2018don}} & \textbf{FWT\cite{diaz2018don}} & \textbf{A\cite{diaz2018don}} & \st{OverallAcc} & \textbf{ACC~\cite{lopez2017gradient}} \\ \hline
EWC            & -95.9683     & 2.1317       & 40.71             & 25.44                & 28.20            \\ \hline
LwF            & -80.1867     & 14.12        & 46.67             & 29.17                & 33.43            \\ \hline
SI             & -95.3733     & 2.7633       & 41.10             & 25.69                & 28.79            \\ \hline
GDumb          & -9.1667      & 82.7         & 82.53             & 51.58                & 79.41            \\ \hline
Replay         & -1.6083      & 96.065       & 96.89             & 60.56                & 96.57            \\ \hline
GEM            & -32.3767     & 63.1967      & 76.51             & 47.82                & 67.20            \\ \hline
Naive          & -97.135      & 0.6733       & 39.74             & 24.84                & 24.97            \\ \hline
Cumulative     & 5.4433       & 96.9467      & 91.52             & 57.20                & 87.40            \\ \hline
Joint  & --            & --            & 86.22             & 86.21                & 86.21            \\ \hline
\end{tabular}
\end{table*}


% \begin{table*}[htbp!]
% \caption{Comparative analysis of different CL approaches for the class incremental scenario.}
%  \label{tab:CIL}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% {\color[HTML]{333333} CL strategy}}                   & {\color[HTML]{333333} \textbf{BWT[Diaz]}} & \textbf{BWT[Lopez]} & \textbf{FWT[Diaz]} & \textbf{FWT[Lopez]} & \textbf{Accuracy\cite{diaz2018don}} & \textbf{Overall avg. acc.} & \textbf{Last row avg. acc.} \\ \hline
% \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{EWC}}   & {\color[HTML]{333333} -95.9683}            & 53.7634             & 2.1317              & 4.7101              & 40.71             & 25.44                      & 28.20                       \\ \hline
% {\color[HTML]{333333} \textbf{LwF}}                           & {\color[HTML]{333333} -80.1867}            & 56.1750             & 14.12               & -5.2546             & 46.67             & 29.17                      & 33.43                       \\ \hline
% {\color[HTML]{333333} \textbf{SI}}                            & {\color[HTML]{333333} -95.3733}            & 53.8594             & 2.7633              & 4.2417              & 41.10             & 25.69                      & 28.79                       \\ \hline
% \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{GDumb}} & {\color[HTML]{333333} -9.1667}             & 73.4035             & 82.7                & -73.9754            & 82.53             & 51.58                      & 79.41                       \\ \hline
% \textbf{Replay}                                               & -1.6083                                    & 79.4513             & 96.065              & -84.3142            & 96.89             & 60.56                      & 96.57                       \\ \hline
% \textbf{GEM}                                                  & -32.3767                                   & 72.6208             & 63.1967             & -56.3395            & 76.51             & 47.82                      & 67.20                       \\ \hline
% \textbf{Naive}                                                & -97.135                                    & 54.2627             & 0.6733              & 5.5244              & 39.74             & 24.84                      & 24.97                       \\ \hline
% \textbf{Cumulative}                                           & 5.4433                                     & 77.7710             & 96.9467             & -85.6671            & 91.52             & 57.20                      & 87.40                       \\ \hline
% \textbf{Joint Training}                                       & 0                                          & 0                   & 0                   & 0                   & 86.22             & 86.21                      & 86.21                       \\ \hline
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old_intro.tex <==
% Machine learning (ML) and deep learning (DL) models can perform well in the given dataset. But when the new dataset came into the picture, they needed to be retrained with the new dataset and they override the new data or task over the old task learned previously. This phenomenon is called catastrophic forgetting\cite{shao2022overcoming}\cite{french1999catastrophic}\cite{mccloskey1989catastrophic}\cite{ratcliff1990connectionist}
% which is quite prevalent in ML and DL models. To overcome this issue we need to use approaches that can remember everything we learned once. In the real world, the data cannot be obtained at once and it usually comes over time. To handle the streaming data, we need a system that can handle the incoming data continuously This can be done by using continual learning \cite{de2021continual,wang2023comprehensive}. Continual learning is an approach that allows the model to learn new data and remember the previous learning simultaneously. Different continual learning approaches are used to handle catastrophic forgetting. We will use a few of them to compare their performance in terms of accuracy. The approaches used are EWC, GEM, SI, LwF, GDumb, Replay, Naive, cumulative, and Joint Training. We have used simple CNN, RESNET50, and RESNET18, as the background models for these approaches in the DCASE audio data.

% audio-based monitoring refers to using audio signals to monitor and analyze various phenomena in diverse environments. The monitoring may require huge manpower if we try it manually and may not be as accurate as required. So to automate the monitoring, we need to use some sensors and machine learning techniques.
% With the expansion of sensor technologies and the increasing availability of audio data, audio-based monitoring has emerged as a powerful tool across numerous domains, including but not limited to security surveillance, environmental monitoring, wildlife conservation, and healthcare. 
% Monitoring can be provided in many ways by using any sort of modalities like audio, video, images, etc, here we have tried to use audio data which is 1-dimensional data that can easily be stored and processed. Unlike traditional monitoring methods, which often rely on visual or physical sensors, audio-based monitoring offers unique advantages, such as non-invasiveness, remote operation, and the ability to capture rich contextual information. Moreover, audio data is easier to acquire and handle than other modalities as it is not affected by illumination unlike image data, does not require any line of sight to the target, and is easy to capture using microphones \cite{vranken2023sound}. 




% \textcolor{blue}{The agriculture supplies food and other resources to society. The agricultural farms include the big spread farms and the smallholder farms. The farms support livestock as well as crop production. We all know agriculture is considered the most important sector that plays a crucial role globally, and the integration of artificial intelligence has emerged as a notable trend in enhancing agricultural intelligence. Monitoring agricultural activities intelligently is a significant component of this development \cite{gao2023building}. To support monitoring the farms, we need to provide surveillance to the farms to protect production and support the country's economy. The monitoring may require huge manpower if we try it manually and may not be as accurate as required. So to automate the surveillance, we need to use some sensors and machine learning techniques. Surveillance can be provided in many ways by using any sort of modalities like audio, video, images, etc, here we have tried to use audio data which is 1-dimensional data that can easily be stored and processed. Audio data is easier to acquire and handle than other modalities as it is not affected by illumination unlike image data, does not require any line of sight to the target, and is easy to capture using microphones \cite{vranken2023sound}. Although our main target is to protect the farms using audio data, as the audio data of the farms are not freely available till now, we are trying to study the DCASE challenge audio data in standard continual learning approaches and compare them based on accuracy and other performance metrics. Further, we will apply those CL approaches to the actual farm data. We are using DCASE data because it is a huge standard source of audio data that is available publicly.}

% \textcolor{blue}{Agricultural farms usually suffer from intrusion. Intrusion can be unauthorized human trespassing or wild animal intrusion \cite{ravi2023cnn} which can harm and destroy the crops and their production. Intrusion detection can be for the farms to monitor the invasion of privacy. Animal intrusion in agricultural farms is a concern as it can damage the crops as well as create a threat-like situation for farmers working on the farms \cite{mamat2022animal}. Intrusion detection can also be done to detect the intrusion in the smart devices (IoT devices) or the sensors used for the farm surveillance \cite{el2023optimized}\cite{kethineni2023intrusion}. In this paper, we are considering the intrusion of animals in farms. The method that can be used to overcome this is the technique of machine learning along with the audio sensor.}

% \textcolor{blue}{Machine learning (ML) and deep learning (DL) models can perform well in the given dataset. But when the new dataset came into the picture, they needed to be retrained with the new dataset and they override the new data or task over the old task learned previously. This phenomenon is called catastrophic forgetting\cite{shao2022overcoming}\cite{french1999catastrophic}\cite{mccloskey1989catastrophic}\cite{ratcliff1990connectionist}
% which is quite prevalent in ML and DL models. To overcome this issue we need to use approaches that can remember everything we learned once. In the real world, the data cannot be obtained at once and it usually comes over time. To handle the streaming data, we need a system that can handle the incoming data continuously This can be done by using continual learning \cite{de2021continual,wang2023comprehensive}. Continual learning is an approach that allows the model to learn new data and remember the previous learning simultaneously. Different continual learning approaches are used to handle catastrophic forgetting. We will use a few of them to compare their performance in terms of accuracy. The approaches used are EWC, GEM, SI, LwF, GDumb, Replay, Naive, cumulative, and Joint Training. We have used simple CNN, RESNET50, and RESNET18, as the background models for these approaches in the DCASE audio data.}

% \textcolor{blue}{There are three fundamental scenarios of continual learning: task-incremental, domain-incremental, and class-incremental learning. Out of them, in this paper, the dataset is arranged in two criteria namely domain incremental and class incremental. In domain incremental, the data consists of data samples in different batches or tasks, and each task has similar classes but a different distribution of data samples. While in class incremental, the tasks can have different classes associated with the data distribution. The continual learning approaches are used to handle this kind of distribution of samples and classes in real data. } 

==> old_literature.tex <==
\section{Literature Review}
Farm surveillance and intrusion detection have been enduring concerns. In the past, conventional approaches involved employing guards for manual safeguarding, utilizing humanoid scarecrows, or installing electric fences around farms. However, the current trend is shifting towards automating surveillance to enhance convenience for farmers, aiming to boost production and contribute to economic growth. In recent years, research has increasingly focused on farm surveillance through the integration of IoT, computer vision, and machine learning methods. The common practices for safeguarding farms against wild animal intrusion involve the use of IoT sensors \cite{bapat2017wsn}\cite{sandeep2022design} \cite{begum2020internet}\cite{angadi2019agrivigilance} such as PIR sensors \cite{mane2022smart} \cite{thakur2020smart}\cite{alui2023prototype}, cameras \cite{sureshkumar2020efficient} \cite{banupriya2020animal} installed in the farms, and video surveillance \cite{singh2020animal} throughout the day. Additionally, some employ RFID \cite{santhiya2018smart}, Arduino \cite{yadahalli2020smart}, or Raspberry Pi \cite{AshokKumar} \cite{kakade2019design} for animal detection on farms. The integration of multimodal approaches, such as combining cameras with audio sensors \cite{anuvind2023development}, has also proven useful for intrusion detection. The literature for intrusion detection is briefly described in table \ref{tab:intrusion detection}.

 Nevertheless, the majority of existing farm surveillance systems are trained on fixed datasets using machine learning (ML) or deep learning (DL) models, lacking the capability to adapt to new data over time. In contrast to ML and DL, continual learning or lifelong learning methods enable machine learning models to learn sequentially from a continuous stream of data. This approach allows them to acquire new skills and accumulate knowledge over time without the risk of forgetting previously learned experiences, as emphasized by \cite{parisi2019continual}.  While not a novel concept, continual learning (CL) is an emerging idea that finds applications in various fields, including anomaly detection \cite{8682702}, medical imaging \cite{quarta2022continual}, audio analysis/classification \cite{9413584} \cite{karam2022task}\cite{muthuchamy2023adapter}\cite{zhang2023remember}\cite{mulimani2024class}, audio captioning \cite{berg2021continual}, audio-visual analysis \cite{Mo_2023_ICCV}\cite{pian2023audio}, speech recognition \cite{sadhu2020continual}, and more. This paper predominantly concentrates on the application of continual learning in the audio domain The literature for different approaches of continual learning is mentioned in table \ref{tab:CL_literature}.

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htbp!]
\caption{Literature for intrusion detection}
\label{tab:intrusion detection}
\scalebox{0.8}{
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{{\color[HTML]{333333} \textbf{Authors}}}                                                 & \multicolumn{1}{c|}{{\color[HTML]{333333} \textbf{Technique}}}                              & {\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}l@{}}Sensing \\ Modality\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Description}}                                                                                                                                       \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Kumar et al. \\ (2022) \cite{venkateshkumar2022farm}\end{tabular}} & {\color[HTML]{333333} Threshold}                                                            & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}PIR, IR \\ sensors\end{tabular}}           & \begin{tabular}[c]{@{}l@{}}Used arduino, LCD display\\ \& Activates buzzer when \\ intrusion detected.\end{tabular}                                                             \\ \hline
{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Tsalera et al. \\ (2021) \cite{tsalera2021comparison}\end{tabular}}                       & {\color[HTML]{333333} CNN}                                                                  & {\color[HTML]{333333} Audio}                                                                & \begin{tabular}[c]{@{}l@{}}Used GoogLeNet, SqueezeNet,\\ ShuffleNet, VGGish \&YAMNet, \\ \& applied transfer learning \& \\ obtaining the last 2 performed better.\end{tabular} \\ \hline
{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Mascarenhas\\  et al.  (2021) \cite{mascarenhas2021comparison}\end{tabular}}                  & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}VGG16, \\ VGG19, \\ ResNet50\end{tabular}} & {\color[HTML]{333333} Image}                                                                & \begin{tabular}[c]{@{}l@{}}Compared 3 methods and obtained\\ ResNet50 shows better accuracy.\end{tabular}                                                                       \\ \hline
{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Sabeenian \\ et al. (2020) \cite{sabeenian2020wild}\end{tabular}}                     & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Machine \\ Learning\end{tabular}}          & {\color[HTML]{333333} Video}                                                                & \begin{tabular}[c]{@{}l@{}}Used camera to monitor farm \& detect\\ animal intrusion \& produce appropriate\\ sounds to drive the animal away.\end{tabular}                      \\ \hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[htbp!]
\caption{Literature for continual learning}
\label{tab:CL_literature}
\scalebox{0.9}{
\begin{tabular}{|l|l|l|l|}

\hline
\multicolumn{1}{|c|}{{\color[HTML]{333333} \textbf{Authors}}}                                                    & \multicolumn{1}{c|}{{\color[HTML]{333333} \textbf{Technique}}}                          & \multicolumn{1}{c|}{\textbf{Dataset}}                           & \multicolumn{1}{c|}{\textbf{Approach}}                                                 \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Ashfahani\\ et al. (2022) \cite{ashfahani2022unsupervised}\end{tabular}} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}CNN, MLP,\\ Auto encoder\end{tabular}} & \begin{tabular}[c]{@{}l@{}}MNIST,\\ CIFAR\end{tabular}          & \begin{tabular}[c]{@{}l@{}}Regularization,\\ Dynamic network\end{tabular}              \\ \hline
{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Gao et al. \\ (2022) \cite{gao2022efficient}\end{tabular}}                              & {\color[HTML]{333333} RNN}                                                              & \begin{tabular}[c]{@{}l@{}}MNIST,\\ CIFAR\end{tabular}          & Dynamic network                                                                        \\ \hline
{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Li et al. \\ (2020) \cite{li2020continual}\end{tabular}}                               & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}BNN, GMM,\\ EM algo\end{tabular}}      & \begin{tabular}[c]{@{}l@{}}MNIST,\\ Time-series\end{tabular}    & Dynamic network                                                                        \\ \hline
\color[HTML]{333333}{\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}Ororbia et al. \\ (2020) \cite{ororbia2020continual}\end{tabular}}  & {\color[HTML]{333333} RNN}                                                              & \begin{tabular}[c]{@{}l@{}}MNIST, Penn \\ treebank\end{tabular} & Memory replay                                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}Sun et al. \\ (2020) \cite{sun2020multimodal}\end{tabular}                                                     & \begin{tabular}[c]{@{}l@{}}Online dictionary\\ updating\end{tabular}                    & LMT                                                             & Dynamic network                                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Derakhshani\\ et al. (2022) \cite{derakhshani2022lifelonger}\end{tabular}                                              & ResNet-18                                                                               & MedMNIST                                                        & \begin{tabular}[c]{@{}l@{}}CL approaches\\ (LwF, MAS, EWC,\\ iCaRL, EEIL)\end{tabular} \\ \hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!htbp]
\centering
\caption{Comparing the state-of-the-art works for audio intrusion detection with the proposed work \textcolor{red}{(rough)}}

% \caption{A summary of related work}
 \label{tab:comp_literature}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Work& \begin{tabular}[c]{@{}c@{}}Research\\ application \end{tabular}  &  \begin{tabular}[c]{@{}c@{}}Learning type \end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Can handle \\ unseen classes? \end{tabular}  &\begin{tabular}[c]{@{}c@{}}Domain shift\\ considered? \end{tabular}  &
 \begin{tabular}[c]{@{}c@{}}Datasets used \end{tabular}   \\\hline
 

 
 Foggia et al.~\cite{foggia2015audio}& \begin{tabular}[c]{@{}c@{}}road monitoring\end{tabular} &  \begin{tabular}[c]{@{}c@{}}static \end{tabular} &no&no& \\\hline
 
xyz et al.~\cite{}& \begin{tabular}[c]{@{}c@{}}public monitoring\end{tabular} &  \begin{tabular}[c]{@{}c@{}}static \end{tabular} &no&no& \\\hline

xyz et al.~\cite{}& \begin{tabular}[c]{@{}c@{}}patient monitoring\end{tabular} &  \begin{tabular}[c]{@{}c@{}}static \end{tabular} &no&no& \\\hline

xyz et al.~\cite{}& \begin{tabular}[c]{@{}c@{}}machine monitoring\end{tabular} &  \begin{tabular}[c]{@{}c@{}}static \end{tabular} &no&no& \\\hline

xyz et al.~\cite{}& \begin{tabular}[c]{@{}c@{}}smart-home monitoring\end{tabular} &  \begin{tabular}[c]{@{}c@{}}static \end{tabular} &no&no& \\\hline

CL approaches&\begin{tabular}[c]{@{}c@{}}-- \end{tabular} & \begin{tabular}[c]{@{}c@{}}continual\end{tabular} &yes&\begin{tabular}[c]{@{}c@{}}yes \end{tabular} & \\\hline

\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

% \textcolor{red}{literature is still in progress.} 
